The isothermal limit for the compressible Euler equations with damping

We consider the isothermal Euler system with damping. We rigorously show the convergence of Barenblatt solutions towards a limit Gaussian profile in the isothermal limit $\gamma$ $\rightarrow$ 1, and we explicitly compute the propagation and the behavior of Gaussian initial data. We then show the weak L 1 convergence of the density as well as the asymptotic behavior of its first and second moments. Contents 1. Introduction 1 2. Assumptions and main results 3 3. The limit $\gamma$ $\rightarrow$ 1 of Barenblatt's solutions 6 4. Gaussian solutions 9 5. Evolution of certain quantities 10 6. Convergence 15 7. Conclusion 17 References 17

==> convergence_rate.tex <==
\section{Proof of the main Theorem}

We multiply equation \eqref{entropy_eq} by a factor $(1+t)^k$ (where $k>0$ is yet to be fixed) so we get
\[ (1+t)^k \frac{d}{dt} \int_{\R} \left( \eta_* (t,x) +  \log( \overline{\rho}) ( \rho -\overline{\rho} ) \right) dx + (1+t)^k \int_{\R} \left( \frac{m^2}{\rho} - \frac{\overline{m}^2}{\overline{\rho}} \right) dx \leq 0, \]
that we can rewrite
\begin{multline*}
 \frac{d}{dt} \int_{\R} (1+t)^k \eta_* (t,x) dx +  (1+t)^k \int_{\R} \left( \frac{m^2}{\rho} - \frac{\overline{m}^2}{\overline{\rho}} \right) dx \\
 \leq  k(1+t)^{k-1} \int_{\R} \eta_* (t,x) dx + (1+t)^k \frac{d}{dt} \int_{\R}  \log( \overline{\rho}) ( \overline{\rho} - \rho)  dx. 
 \end{multline*}
Integrating the above over $\left[0,t\right]$, we have
\begin{multline} \label{big_inequality}
(1+t)^k \int_{\R}  \eta_* (t,x) dx +   \int_0^t \int_{\R} (1+s)^k \left( \frac{m^2}{\rho} - \frac{\overline{m}^2}{\overline{\rho}} \right) dx ds \\
\leq C + \int_0^t  \int_{\R} k(1+s)^{k-1}\eta_* (s,x) dx ds +  \int_0^t (1+s)^k  \frac{d}{dt} \int_{\R} \log( \overline{\rho}) ( \overline{\rho} - \rho)  dx ds,
 \end{multline}
where $C>$ stands as a generic constant independent of $(t,x)$ through the rest of the proof. We are now going to study each of these terms separately. \\

First off, recalling that
\[ P(\rho) - P(\overline{\rho}) - P'(\overline{\rho}) (\rho-\overline{\rho}) =  \rho \log \left( \frac{\rho}{\overline{\rho}}   \right) + \overline{\rho} - \rho, \]
and as we took $\overline{\rho}_0$ such that 
\[  \int_{\R} \rho = \int_{\R} \rho_0 = \int_{\R} \overline{\rho}_0 = \int_{\R} \overline{\rho},  \]
we see that
\[  \int_{\R}  \eta_* (t,x) dx =  \int_{\R} \frac{m^2}{\rho} dx + \int_{\R} \rho \log \left( \frac{\rho}{\overline{\rho}}   \right) \geq \int_{\R} \rho \log \left( \frac{\rho}{\overline{\rho}}   \right). \]
By the Csiszár-Kullback inequality (see e.g. \cite{ineg_sobo_log}) , we have
\[  \| \rho - \overline{\rho} \|^2_{L^1(\R)} \leq 2 \| \rho_0 \|_{L^1(\R)}  \int_{\R} \rho \log \left( \frac{\rho}{\overline{\rho}}\right),  \]
so finally
\[  \| \rho - \overline{\rho} \|^2_{L^1(\R)} \lesssim  \int_{\R}  \eta_* (t,x) dx.  \]

For the second integral in the inequality \eqref{big_inequality}, following \cite{marcati2005}, we denote
\[ Q = \frac{ m^2}{\rho} - 2 \frac{\overline{m}}{\overline{\rho}} m + \frac{ \overline{m}^2}{\overline{\rho}} \rho = \left( \frac{m}{\sqrt{\rho}}- \frac{\overline{m}}{\overline{\rho}} \rho \right)^2 \geq 0,  \]
and we remark that
\[  \frac{m^2}{\rho} - \frac{\overline{m}^2}{\overline{\rho}} = 2 \frac{\overline{m}}{\overline{\rho}} (m - \overline{m} ) - \frac{\overline{m}^2}{\overline{\rho}^2} (\rho - \overline{\rho}) +Q.   \]

From the previous section we know that
\[ \frac{\overline{m}(t,x)}{\overline{\rho}(t,x)}= \frac{\dot{r}(t)}{r(t)} x,    \]
and we make the assumption that
\[ \boxed{\left| \int_{\R} y^2(R - \Gamma ) dy \right| \lesssim \frac{1}{\tau(t)} \ \ \ \text{\and} \ \ \ \left| \int_{\R} yM dy \right| \lesssim  \frac{1}{\tau(t)} .} \]
Now we compute
\begin{align*}
    \int_0^t \int_{\R} (1+s)^k \int_{\R} \frac{\overline{m}(s,x)^2}{\overline{\rho}(s,x)^2} (\rho(s,x)-\overline{\rho}(s,x)) dx ds & =  \int_0^t \int_{\R} (1+s)^k \dot{\tau}(s)^2 \int_{\R} \frac{x^2}{\tau(s)^2}  (\rho(s,x)-\overline{\rho}(s,x)) dx ds \\
    & =  \int_0^t \int_{\R} (1+s)^k \dot{\tau}(s)^2 \int_{\R} y^2 (R - \Gamma ) dy ds \\
    & \leq \int_0^t (1+s)^k \frac{\dot{\tau}(s)^2}{\tau(s)} ds \\
    & \lesssim (1+t)^{k-1/2},
\end{align*}
and
\begin{align*}
    \int_0^t \int_{\R} (1+s)^k \int_{\R} \frac{\overline{m}(s,x)}{\overline{\rho}(s,x)} (m(s,x)-\overline{m}(s,x)) dx ds & = \int_0^t \int_{\R} (1+s)^k  \dot{\tau}(s) \int_{\R} \frac{x}{\tau(s)}  (m(s,x)-\overline{m}(s,x)) dx ds \\
    & = \int_0^t \int_{\R} (1+s)^k  \frac{\dot{\tau}(s)}{\tau(s)} \int_{\R} y M dy ds + \int_0^t (1+s)^k \dot{\tau}(s)^2 \int_{\R} y^2(R - \Gamma) dy ds \\
   & \leq  \int_0^t (1+s)^k \frac{\dot{\tau}(s)}{\tau(s)^2} ds + \int_0^t (1+s)^k \frac{\dot{\tau}(s)^2}{\tau(s)} ds \\
    & \lesssim (1+t)^{k-1/2}.
\end{align*}


For the first term, we recall that 
\[ \eta_* = \rho \log \left( \frac{\rho}{\overline{\rho}} \right) + \frac{m^2}{\rho}.  \]
From the energy equality \eqref{eq_energy} , writing $k=1- \eps$ with $0 < \eps < 1 $, we get that
\[ \sup_{t\geq 0} \int_0^t \frac{1}{(1+s)^{\eps}}\int_{\R} \frac{m^2}{\rho} dx ds \leq C.    \]
We now need to estimate
\[  \int_0^t \int_{\R} (1+s)^{k-1} \int_{\R} \rho(s,x) \log \left( \frac{\rho(s,x)}{\overline{\rho}(s,x)} \right) dx ds  = \int_0^t \int_{\R} \frac{1}{(1+s)^{\eps}} \int_{\R} R \log \left( \frac{R}{\Gamma}  \right) dy ds .
\]


For the second term, we write
\begin{multline*}
\int_0^t (1+s)^k \frac{d}{dt} \int_{\R} \log(\overline{\rho}) (\overline{\rho}-\rho) \\
= C(\rho_0,\overline{\rho}_0) + (1+t)^k \int_{\R} \log( \overline{\rho}(t,x)) (\overline{\rho}(t,x)-\rho(t,x)) dx -  \int_0^t k(1+s)^{k-1} \int_{\R} \log(\overline{\rho}) (\rho - \overline{\rho})dxds.     
\end{multline*} 
With the previous notations, we write
\[ - \int_0^t (1+s)^{k-1} \frac{d}{dt} \int_{\R} \log(\overline{\rho}(s,x)) (\overline{\rho}(s,)-\rho(s,x)) dx ds = \int_0^t (1+s)^{k-1} \int_{\R} \log( \Gamma ) (R- \Gamma) dy ds \lesssim  (1+t)^{k-1/2}. \]
